Sometimes the Model doth Preach: Quantifying Religious Bias in Open LLMs through Demographic Analysis in Asian Nations

Large Language Models (LLMs) are capable of generating opinions and propagating bias unknowingly, originating from unrepresentative and non-diverse data collection. Prior research has analysed these opinions with respect to the West, particularly the United States. However, insights thus produced may not be generalized in non-Western populations. With the widespread usage of LLM systems by users across several different walks of life, the cultural sensitivity of each generated output is of crucial interest. Our work proposes a novel method that quantitatively analyzes the opinions generated by LLMs, improving on previous work with regards to extracting the social demographics of the models. Our method measures the distance from an LLM's response to survey respondents, through Hamming Distance, to infer the demographic characteristics reflected in the model's outputs. We evaluate modern, open LLMs such as Llama and Mistral on surveys conducted in various global south countries, with a focus on India and other Asian nations, specifically assessing the model's performance on surveys related to religious tolerance and identity. Our analysis reveals that most open LLMs match a single homogeneous profile, varying across different countries/territories, which in turn raises questions about the risks of LLMs promoting a hegemonic worldview, and undermining perspectives of different minorities. Our framework may also be useful for future research investigating the complex intersection between training data, model architecture, and the resulting biases reflected in LLM outputs, particularly concerning sensitive topics like religious tolerance and identity.

==> Profiles.tex <==
\subsection{Appendix A: Model Profiles across Countries}

\FloatBarrier

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{EA-modelProfiles/HKG.jpg}
    \caption{Model Profiles - Hong Kong}
    \label{fig:hkg-profiles}
\end{figure*}

\clearpage

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{EA-modelProfiles/KOR1.jpg}
    \caption{Model Profiles - Korea (Part 1 of 2)}
    \label{fig:kor-profiles}
\end{figure*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{EA-modelProfiles/KOR2.jpg}
    \caption{Model Profiles - Korea (Part 2 of 2)}
\end{figure*}

\clearpage


\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{EA-modelProfiles/TWN1.jpg}
    \caption{Model Profiles - Taiwan (Part 1 of 2)}
    \label{fig:twn-profiles}
\end{figure*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{EA-modelProfiles/TWN2.jpg}
    \caption{Model Profiles - Taiwan (Part 2 of 2)}
\end{figure*}

\clearpage

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{EA-modelProfiles/VNM.jpg}
    \caption{Model Profiles - Vietnam}
    \label{fig:vnm-profiles}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{SEA_modelProfiles/MYS.jpg}
    \caption{Model Profiles - Malaysia}
    \label{fig:mys-profiles}
\end{figure*}

\clearpage

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{SEA_modelProfiles/KHM.jpg}
    \caption{Model Profiles - Cambodia}
    \label{fig:khm-profiles}
\end{figure*}

\clearpage

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{SEA_modelProfiles/SGP.jpg}
    \caption{Model Profiles - Singapore}
    \label{fig:sgp-profiles}
\end{figure*}

\clearpage

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{SEA_modelProfiles/LKA.jpg}
    \caption{Model Profiles - Sri Lanka}
    \label{fig:lka-profiles}
\end{figure*}

\clearpage

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{SEA_modelProfiles/THA.jpg}
    \caption{Model Profiles - Thailand}
    \label{fig:khm-profiles}
\end{figure*}

\clearpage




==> annexure.tex <==
\subsection{Results}

\begin{table}[htbp]
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{Model}           & \multicolumn{1}{c|}{Profile}                                  \\ \hline
\multirow{7}{*}{Llama 3.1 (Base)} & Most likely Hindu, Male (57.5\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (\%)           \\ \cline{2-2} 
                                      & Within 18-25 years of age. (50\%)                             \\ \cline{2-2} 
                                      & Married (78.6\%), 2 Children (35.7\%), at least 1 daughter (54.6\%) \\ \cline{2-2} 
                                      & Lives in Rural (53.9\%), North India (32.5\%).                    \\ \cline{2-2} 
                                      & Has a High school; Industrial training
                                      institute Degree  (20.9\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of \textless Rs. 10k (51.0\%)         \\ \hline
\multirow{7}{*}{Llama 3.1 (Instruct)} & Most likely Hindu, Male (58\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (48.9\%)           \\ \cline{2-2} 
                                      & Within 26-34 years of age (26.7\%)                              \\ \cline{2-2} 
                                      & Married (78.1\%), 2 Children (34.5\%), at least 1 daughter (53.7\%) \\ \cline{2-2} 
                                      & Lives in Rural (53\%),  West (40.4\%)                    \\ \cline{2-2} 
                                      & Upper primary (upper primary certificate) (20.1\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of \textless Rs. 10k  (50.5\%)          \\ \hline
\end{tabular}%
}
\label{tbl:profiles-llama}
\caption{Model Profile of Llama 3.1 Models}
\end{table}


\begin{table}[htbp]
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{Model}           & \multicolumn{1}{c|}{Profile}                                  \\ \hline
\multirow{7}{*}{Llama 3.2 (Instruct)} & Most likely Hindu, Male (59\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (53\%)           \\ \cline{2-2} 
                                      & Within 35-44 years of age. (29\%)                             \\ \cline{2-2} 
                                      & Married (82\%), 2 Children (37\%), at least 1 daughter (56\%) \\ \cline{2-2} 
                                      & Lives in Rural (56\%), North India (38\%).                    \\ \cline{2-2} 
                                      & May be a Senior Secondary School Graduate (38\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of  \textless Rs. 10k (43\%)         \\ \hline
\multirow{7}{*}{Llama 3.2 (Base)}     & Most likely Hindu, Male (59\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (52\%)           \\ \cline{2-2} 
                                      & Within 35-44 years of age (28\%)                              \\ \cline{2-2} 
                                      & Married (80\%), 2 Children (36\%), at least 1 daughter (56\%) \\ \cline{2-2} 
                                      & Lives in Rural (55\%),  North India (33\%)                    \\ \cline{2-2} 
                                      & May be a Senior Secondary School Graduate (40\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of \textless Rs. 10k (47\%)          \\ \hline
\end{tabular}%
}
\label{tbl:profiles-llama}
\caption{Model Profile of Llama 3.2 Models}
\end{table}

\begin{table}[htbp]
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{Model}           & \multicolumn{1}{c|}{Profile}                                  \\ \hline
\multirow{7}{*}{Gemma 7B (Base)} & Most likely Hindu, Male (59\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (53\%)           \\ \cline{2-2} 
                                      & Within 35-44 years of age. (26\%)                             \\ \cline{2-2} 
                                      & Married (77.1\%), 2 Children (34.6\%), at least 1 daughter (52.8\%) \\ \cline{2-2} 
                                      & Lives in Urban (57\%), North India (38.8\%).                    \\ \cline{2-2} 
                                      & Has a High school; Industrial training
                                      institute Degree  (20.4\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of  Rs. 10k (48.6\%)         \\ \hline
\multirow{7}{*}{Gemma 7B (Instruct)} & Most likely Hindu, Male (58.6\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (48.5\%)           \\ \cline{2-2} 
                                      & Within 35-44 years of age (30.1\%)                              \\ \cline{2-2} 
                                      & Married (81.6\%), 2 Children (37.7\%), at least 1 daughter (56.3\%) \\ \cline{2-2} 
                                      & Lives in Rural (57.3\%),  North India (52.6\%)                    \\ \cline{2-2} 
                                      & Has a High school; Industrial training
                                      institute Degree (24.9\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of  Rs. 10k and Above (51.1\%)          \\ \hline
\end{tabular}%
}
\label{tbl:profiles-llama}
\caption{Model Profile of Gemma 7B Models}
\end{table}

\begin{table}[htbp]
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{Model}           & \multicolumn{1}{c|}{Profile}                                  \\ \hline
\multirow{7}{*}{Gemma 2 9B (Base)} & Most likely Hindu, Male (58.9\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (48.1\%)           \\ \cline{2-2} 
                                      & Within 35-44 years of age. (26.5\%)                             \\ \cline{2-2} 
                                      & Married (77.2\%), 2 Children (35.5\%), at least 1 daughter (53.6\%) \\ \cline{2-2} 
                                      & Lives in Rural (57.8\%), North India (39.4\%).                    \\ \cline{2-2} 
                                      & Has a High school; Industrial training
                                      institute Degree  (21.2\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of \textless Rs. 10k (48.2\%)         \\ \hline
\multirow{7}{*}{Gemma 2 9B (Instruct)} & Most likely Hindu, Male (69.9\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (40.1\%)           \\ \cline{2-2} 
                                      & Within 18-25 years of age (28.2\%)                              \\ \cline{2-2} 
                                      & Married (72.7\%), 2 Children (31.5\%), at least 1 daughter (46.5\%) \\ \cline{2-2} 
                                      & Lives in Rural (64\%),  North India (33.6\%)                    \\ \cline{2-2} 
                                      & Upper primary (upper primary certificate) (20.9\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of \textless Rs. 10k  (52.1\%)          \\ \hline
\end{tabular}%
}
\label{tbl:profiles-llama}
\caption{Model Profile of Gemma 2 9B Models}
\end{table}

\begin{table}[htbp]
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{Model}           & \multicolumn{1}{c|}{Profile}                                  \\ \hline
\multirow{7}{*}{Mistral 7B v0.1 (Base)} & Most likely Hindu, Male (60.7\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (48.8\%)           \\ \cline{2-2} 
                                      & Within 35-44 years of age. (27.2\%)                             \\ \cline{2-2} 
                                      & Married (77.1\%), 2 Children (36.2\%), at least 1 daughter (53.7\%) \\ \cline{2-2} 
                                      & Lives in Rural (56.2\%), North India (39.4\%).                    \\ \cline{2-2} 
                                      & Has a High school; Industrial training
                                      institute Degree  (21.6\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of \textless Rs. 10k (49.6\%)         \\ \hline
\multirow{7}{*}{Mistral 7B v0.1 (Instruct)} & Most likely Hindu, Male (62.6\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (49.1\%)           \\ \cline{2-2} 
                                      & Within 26-34 years of age. (30\%)                             \\ \cline{2-2} 
                                      & Married (81.8\%), 2 Children (35.5\%), at least 1 daughter (57.3\%) \\ \cline{2-2} 
                                      & Lives in Rural (62.5\%), North India (50.5\%).                    \\ \cline{2-2} 
                                      & Has a High school; Industrial training
                                      institute Degree  (20.9\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of \textless Rs. 10k (40.5\%)         \\ \hline                                      
\multirow{7}{*}{Mistral 7B v0.3 (Base)} & Most likely Hindu, Male (59.3\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (48.4\%)           \\ \cline{2-2} 
                                      & Within 35-44 years of age (26.2\%)                              \\ \cline{2-2} 
                                      & Married (76.3\%), 2 Children (35.2\%), at least 1 daughter (53.1\%) \\ \cline{2-2} 
                                      & Lives in Rural (58.3\%),  North India (36.7\%)                    \\ \cline{2-2} 
                                      & Upper primary (upper primary certificate) (21.6\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of \textless Rs. 10k  (49.1\%)          \\ \hline
\multirow{7}{*}{Mistral 7B v0.3 (Instruct)} & Most likely Hindu, Male (58.9\%).                               \\ \cline{2-2} 
                                      & Most likely member from the General Category (47.6\%)           \\ \cline{2-2} 
                                      & Within 26-34 years of age (30.8\%)                              \\ \cline{2-2} 
                                      & Married (81\%), 2 Children (34.5\%), at least 1 daughter (54.5\%) \\ \cline{2-2} 
                                      & Lives in Rural (59.4\%),  North India (44.4\%)                    \\ \cline{2-2} 
                                      & Has a High school; Industrial training
                                      institute Degree (20.4\%)              \\ \cline{2-2} 
                                      & Monthly Household Income of \textless Rs. 10k  (43.7\%)          \\ \hline
\end{tabular}%
}
\label{tbl:profiles-llama}
\caption{Model Profile of Mistral Models}
\end{table}

==> eaSurvey.tex <==
\subsection{Appendix C: Demographics in EA Survey}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{EA/HKG1.png}
    \caption{Number of Survey Respondents per Demographic Variable - Hong Kong (Part 1 of 2)}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{EA/HKG2.png}
    \caption{Number of Survey Respondents per Demographic Variable - Hong Kong (Part 2 of 2)}
\end{figure}

\clearpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{EA/JPN1.png}
    \caption{Number of Survey Respondents per Demographic Variable - Japan (Part 1 of 2)}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{EA/JPN2.png}
    \caption{Number of Survey Respondents per Demographic Variable - Japan (Part 2 of 2)}
\end{figure}

\clearpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{EA/KOR1.png}
    \caption{Number of Survey Respondents per Demographic Variable - South Korea (Part 1 of 2)}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{EA/KOR2.png}
    \caption{Number of Survey Respondents per Demographic Variable - South Korea (Part 2 of 2)}
\end{figure}

\clearpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{EA/TWN1.png}
    \caption{Number of Survey Respondents per Demographic Variable - Taiwan (Part 1 of 3)}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{EA/TWN2.png}
    \caption{Number of Survey Respondents per Demographic Variable - Taiwan (Part 2 of 3)}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{EA/TWN3.png}
    \caption{Number of Survey Respondents per Demographic Variable - Taiwan (Part 3 of 3)}
\end{figure}

\clearpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{EA/VNM1.png}
    \caption{Number of Survey Respondents per Demographic Variable - Vietnam (Part 1 of 2)}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{EA/VNM2.png}
    \caption{Number of Survey Respondents per Demographic Variable - Vietnam (Part 2 of 2)}
\end{figure}

==> indiaSurvey.tex <==
\subsection{Appendix B: Demographics in India Survey}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{india_demo_1.png}
    \caption{Number of Survey Respondents per Demographic Variable in Indian Survey (part 1 of 2).}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{india_demographic_2.png}
    \caption{Number of Survey Respondents per Demographic Variable in Indian Survey (part 2 of 2).}
\end{figure}



==> old.tex <==
\section{Dataset}

Our current experiments are two-fold, we have ourselves prepared a dataset comprised of questions from a Pew Research Survey on Gender and Religious Tolerance \cite{indiaSurvey} - and have also used some of the existing OpinionQA dataset to look into potential trends/changing alignments with a newer generation of Large Language Models.

\subsection{India Survey Data}

The Survey Dataset we had selected reports on 29,999 Indian adults about various aspects about religion in their day-to-day life and its tolerance in Indian society. The survey provides us a total of 87 questions which may or may not contain more than one sub-question, closely related to the main question itself. Each question can only have one answer, however, the number of options per question may vary with the question.

We manually selected 19 questions, on the basis of which questions directly probed with social phenomena such as Women's Rights, Religion, etc, as compared to those which probed the demographic of the respondent instead.

\subsection{OpinionQA}

At the time of publication of the original work, Large Language Models that were available for study consisted mainly of the GPT-3 family of models, such as text-davinci, ada, etc. Since then, along with the drastic increase in number of parameters in the GPT-4 family and also newer models such as o1, a newer paradigm of open models has also emerged. Models such as Gemma, Llama and Mistral fall under this category, freely available models that can easily be customized to suit particular requirements and whose code and training data is available for us for inspection.

This development motivates the assessment of the newer models on the previous, existing dataset. While analysing our models on data from the OpinionQA dataset, we limited ourselves to questions and responses from a single survey; whereas the previous work considered a total of 15 surveys.

\section{Methodology}

In the previous work by Santurkar et al., the model opinion distribution is extracted by fetching the log-probabilities of the options having provided an appropriate prompt. We replicate this in our experiments.

We also retain the prompting strategies used in steering the LLM, that is:

\begin{enumerate}
	\item QA; where the group information is presented as a multiple-choice question.
	\item BIO; where the information is provided in a free-text manner.
	\item PORTRAY; where the model is instructed to pretend to be a member of a particular group.
\end{enumerate}

\subsection{India Survey Data}

Our experiments prompt our selected models to respond as though they belonged to a particular religion, specifically whether they were a Hindu, Muslim, Christian, Sikh, Buddhist, Jain or Parsi, as these were the options provided in the survey selected by us.

\subsection{OpinionQA}

The previous work prompts on various demographics including race, political ideology, etc. For our experiments so far, we have only prompted the models based on political ideology, that is, we request the model to respond as though they were a Republican, Democrat or Independent.

\subsection{Model Setup}

The following models have been used so far in carrying out our experiments, noted in Table 1.


\begin{table}[htbp]
\centering
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|c|}{Model Name} & \multicolumn{1}{c|}{Number of Parameters} & \multicolumn{1}{c|}{Quantization Configuration} \\ \hline
LLaMA 3                          & 8B                                        & 4-Bit                                           \\ \hline
LLaMA 3.1                        & 8B                                        & 4-Bit                                           \\ \hline
LLaMA 3.2                        & 3B                                        & None                                              \\ \hline
Mistral v0.1                     & 7B                                        & 4-Bit                                           \\ \hline
Mistral v0.3                     & 7B                                        & 4-Bit                                           \\ \hline
Gemma                            & 7B                                        & 4-Bit                                           \\ \hline
Gemma 2                          & 9B                                        & 4-Bit                                           \\ \hline
Falcon                           & 7B                                        & 4-Bit                                           \\ \hline
Falcon                           & 11B                                       & 4-Bit                                           \\ \hline
\end{tabular}
\caption{Models Used}
\end{table}

As detailed in the previous work, the model's opinion distribution is obtained by passing the prompt through the LM and accessing the log-probabilities of the next token being any of the options. As the distribution is obtained from token level log-probabilities, these are expected to be deterministic for any specific prompt, and is independent of the model's random states. 

In our experiments, we have only taken into consideration the top 100 tokens while searching for the option, and in case any particular option is not found within the same, we give that option a zero probability.
  
\section{Results}

\subsection{India Survey Data}

We first compared the distributions obtained from different models with the entire human responses data, to note how close the model responses matched the general consensus opinion of the respondents. As these models are trained on large amounts of internet data, of which the majority is expected to be that of Western, English speaking users, this can also be used as a measure of how close the Indian world-view matches a more global one. The data has been recorded in Table 2 and in Figure 1.

\begin{table}[htbp]
\centering
\begin{tabular}{|l|l|l|l|}
\hline
Model        & Q9     & Q17a   & Q17b   \\ \hline
LLaMA 3      & 0.7585 & 0.7486 & 0.6947 \\ \hline
Mistral v0.1 & 0.9721 & 0.8250 & 0.7607 \\ \hline
\end{tabular}
\caption{Closeness to Human Responses for Select Questions from the Dataset}
\end{table}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.75\linewidth]{questionwise\_closeness.png}
    \caption{Measuring Closeness to Human Responses for LLaMA 3}
    \label{fig:enter-label}
\end{figure}

We note that the model generally reports a high average closeness of 0.7-0.9, with the exception of question 11y, and its seven corresponding sub-questions. Upon examination, we note this to be a question on the perceived level of discrimination against a particular religious community. This discrepancy may be a result of either or both of the following - a misrepresentation on part of the survey respondents under-stating the extent of this issue, or as a result of general Internet discourse exacerbating the topic beyond the actual ground reality. (Speculation.)

\begin{table}[htbp]
\centering
\begin{minipage}{0.45\textwidth}
    \centering
    \begin{tabular}{|l|l|}
    \hline
    \multicolumn{1}{|c|}{Religion} & \multicolumn{1}{c|}{Alignment} \\ \hline
    Buddhist                       & 0.7329                         \\ \hline
    Christian                      & 0.7630                         \\ \hline
    Hindu                          & 0.7251                         \\ \hline
    Jain                           & 0.7120                         \\ \hline
    Muslim                         & 0.7334                         \\ \hline
    Sikh                           & 0.7162                         \\ \hline
    \end{tabular}
    \caption{Alignment Values for LLaMA 3}
\end{minipage}%
\hspace{0.05\textwidth}
\begin{minipage}{0.45\textwidth}
    \centering
    \begin{tabular}{|l|l|}
    \hline
    \multicolumn{1}{|c|}{Religion} & \multicolumn{1}{c|}{Steerability} \\ \hline
    Buddhist                       & 0.8255                            \\ \hline
    Christian                      & 0.8276                            \\ \hline
    Hindu                          & 0.7692                            \\ \hline
    Jain                           & 0.7892                            \\ \hline
    Muslim                         & 0.7850                            \\ \hline
    Sikh                           & 0.8075                            \\ \hline
    \end{tabular}
    \caption{Steerability Values for LLaMA 3}
\end{minipage}
\end{table}

On computing alignment over all questions in our dataset, we noted the results as in Table 3. Correspondingly, we report steerability over the three methods discussed earlier in Table 4.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{alignment_llama_ind.png}
    \caption{Comparing group-wise alignment over the LLaMA 3 family of models.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{steerability_llama_ind.png}
    \caption{Comparing steerability over the LLaMA 3 family of models.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{alignment_gemma_ind.png}
    \caption{Comparing alignment over the Gemma family of models.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{steerability_gemma_ind.png}
    \caption{Comparing steerability over the Gemma family of models.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{alignment_mistral_ind.png}
    \caption{Comparing alignment over the Mistral family of models.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{steerability_mistral_ind.png}
    \caption{Comparing steerability over the Mistral family of models.}
    \label{fig:enter-label}
\end{figure}

We note that the steerability methods have allowed the model response to be better aligned to any particular group, especially so in the case of steering the model to respond as a Christian. This is a pattern reinforced by the introduction of several other models, which need not necessarily even belong to the same family. We report the variation in alignment and steerability across models belonging to the same model family in figures 2 through 6.

\subsection{OpinionQA}

We have here used a single survey from the earlier study, and steer on the basis of political ideology; whether the model or respondent is a Democrat, Republican or an Independent.

We report the variation of alignment and steerability across the various models selected in figures 8 through 13.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{alignment_llama_opinionqa.png}
    \caption{LLaMA 3 Alignment - OpinionQA data}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{steerability_llama_opinionqa.png}
    \caption{LLaMA 3 Steerability - OpinionQA data}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{alignment_gemma_opinionqa.png}
    \caption{Gemma Alignment - OpinionQA data}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{steerability_gemma_opinionqa.png}
    \caption{Gemma Steerability - OpinionQA data}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{alignment_mistral_opinionqa.png}
    \caption{Mistral Alignment - OpinionQA data}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{steerability_mistral_opinionqa.png}
    \caption{Mistral Steerability - OpinionQA data}
    \label{fig:enter-label}
\end{figure}

\section{Future Work}

As of writing the report, we are yet to evaluate model responses based on surveys outside of the Indian context. In addition to this, we have also opted to design our own metric to evaluate alignment and steering, based on computing the Hamming distance between the model response and each individual respondent - following which we extract the common, most frequent demographic details of the closest responses. (See Figure 14.)

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.5\linewidth]{HammingDistanceForOpinions.png}
    \caption{New method to measure alignment based on Hamming Distance}
    \label{fig:enter-label}
\end{figure}

\bibliography{citations}



==> seaSurvey.tex <==
\subsection{Appendix D: Demographics in SEA Survey}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/KHM1.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Cambodia (Part 1 of 2)}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/KHM2.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Cambodia (Part 2 of 2)}
\end{figure}

\clearpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/IDN1.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Indonesia (Part 1 of 2)}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/IDN2.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Indonesia (Part 2 of 2)}
\end{figure}

\clearpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/MYS1.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Malaysia (Part 1 of 2)}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/MYS2.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Malaysia (Part 2 of 2)}
\end{figure}

\clearpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/SGP1.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Singapore (Part 1 of 2)}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/SGP2.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Singapore (Part 2 of 2)}
\end{figure}

\clearpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/LKA1.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Sri Lanka (Part 1 of 2)}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/LKA2.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Sri Lanka (Part 2 of 2)}
\end{figure}

\clearpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/THA1.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Thailand (Part 1 of 2)}
\end{figure}

\newpage

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{SEA-tables/THA2.jpg}
    \caption{Number of Survey Respondents per Demo-
graphic Variable - Thailand (Part 2 of 2)}
\end{figure}



